Multi-step planning with learned effects of partial action executions

In this paper, we propose a novel affordance model, which combines object, action, and effect information in the latent space of a predictive neural network architecture that is built on Conditional Neural Processes. Our model allows us to make predictions of intermediate effects expected to be obtained during action executions and make multi-step plans that include partial actions. We first compared the prediction capability of our model using an existing interaction data set and showed that it outperforms a recurrent neural network-based model in predicting the effects of lever-up actions. Next, we showed that our model can generate accurate effect predictions for other actions, such as push and grasp actions. Our system was shown to generate successful multi-step plans to bring objects to desired positions using the traditional A* search algorithm. Furthermore, we realized a continuous planning method and showed that the proposed system generated more accurate and effective plans with sequences of partial action executions compared to plans that only consider full action executions using both planning algorithms.

==> additional.tex <==
\begingroup
\begin{table}[thbp]
\tbl{n-step prediction errors, results from our experiments.}
{\begin{tabular}{|c|c|c|} \hline
 & \textbf{Sp-Truth}& \textbf{Im-CNN}\\\hline
\textbf{1-step (cm)} & $0.354 \pm 0.072$ & $0.340 \pm 0.044$ \\\hline
\textbf{2-step (cm)} & $0.390 \pm 0.061$  & $0.352 \pm 0.046$ \\\hline
\textbf{3-step (cm)} & $0.417 \pm 0.053$  & $0.364 \pm 0.049$ \\\hline
\textbf{4-step (cm)} & $0.445 \pm 0.046$  & $0.375 \pm 0.051$ \\\hline
\textbf{5-step (cm)} & $0.474 \pm 0.039$  & $0.387 \pm 0.054$ \\\hline
\end{tabular}}
\label{table:cnmp_n_step_errors}
\end{table}
\endgroup


==> captions/Figure_1_caption.tex <==
An overview of the proposed model. Given object image and action or effect information at any time-point, our system can generate the effect trajectory and action execution trajectory.

==> captions/Figure_2_caption.tex <==
Scene showing the parameters of a push action around an object.

==> captions/Figure_3_captions.tex <==
Example lever-up action in the simulator, reused with permission from \cite{seker2019deep}.

==> captions/Figure_4_caption.tex <==
N-step error plots obtained in the LSTM approach, reused with permission \cite{seker2019deep}.

==> captions/Figure_5_caption.tex <==
Results of applying the model's predicted actions in a scene. Images are ordered from left to right. The top row is from the first action execution, the bottom row is from the second action execution. The blue object denotes the target position, the red object is generated from the robot's effect predictions. The blue and red objects are not interactable by the robot. The green object is interactable and is acted upon by the robot, to show the ground truth results of the robot's predicted actions.

==> captions/Figure_6_caption.tex <==
Results of applying push actions on objects on a fixed location with fixed size with different settings.

==> captions/Table_1_caption.tex <==
N-step prediction errors obtained in our model.

==> captions/Table_2_caption.tex <==
Single grasp action prediction results on variable sized objects placed on a fixed location.

==> tables/Table_1.tex <==
\begin{table}
\tbl{N-step prediction errors obtained in our model.}
{\begin{tabular}{|c|c|} \hline
\textbf{1-step (cm)} &  $0.340 \pm 0.044$ \\\hline
\textbf{2-step (cm)} & $0.352 \pm 0.046$ \\\hline
\textbf{3-step (cm)} &  $0.364 \pm 0.049$ \\\hline
\textbf{4-step (cm)} &  $0.375 \pm 0.051$ \\\hline
\textbf{5-step (cm)} &  $0.387 \pm 0.054$ \\\hline
\end{tabular}}
\label{table:Table_1}
\end{table}

==> tables/Table_2.tex <==
\begin{table}
\tbl{Single grasp action prediction results on variable sized objects placed on a fixed location.}
{\begin{tabular}{|c|c|c|c|c|} \hline
\textbf{Error (m)}& \textbf{True}& \textbf{True}& \textbf{False}& \textbf{False} \\
 & \textbf{Positive (\%)} & \textbf{Negative (\%)} & \textbf{Positive (\%)} & \textbf{Negative (\%)} \\\hline
\textbf{$0.275 \pm 0.044$} & 75.17 & 90.48 & 9.52 & 24.82 \\\hline
\end{tabular}}
\label{table:Table_2}
\end{table}
